Online deforestation detection

Deforestation detection using satellite images can make an important contribution to forest management. Current approaches can be broadly divided into those that compare two images taken at similar periods of the year and those that monitor changes by using multiple images taken during the growing season. The CMFDA algorithm described in Zhu et al. (2012) is an algorithm that builds on the latter category by implementing a year-long, continuous, time-series based approach to monitoring images. This algorithm was developed for 30m resolution, 16-day frequency reflectance data from the Landsat satellite. In this work we adapt the algorithm to 1km, 16-day frequency reflectance data from the modis sensor aboard the Terra satellite. The CMFDA algorithm is composed of two submodels which are fitted on a pixel-by-pixel basis. The first estimates the amount of surface reflectance as a function of the day of the year. The second estimates the occurrence of a deforestation event by comparing the last few predicted and real reflectance values. For this comparison, the reflectance observations for six different bands are first combined into a forest index. Real and predicted values of the forest index are then compared and high absolute differences for consecutive observation dates are flagged as deforestation events. Our adapted algorithm also uses the two model framework. However, since the modis 13A2 dataset used, includes reflectance data for different spectral bands than those included in the Landsat dataset, we cannot construct the forest index. Instead we propose two contrasting approaches: a multivariate and an index approach similar to that of CMFDA.

==> 3_Methodology/gridSearchAll_consecFix_cv_mahl.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Thu Mar  9 20:24:52 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{lcl|ccccc}
 site & threshold & variable & 2 & 3 & 4 & 5 & 6 \\ 
  \hline
all & 17.24 & Mahl. dist. & 17.24 & 17.24 & 17.24 & 17.24 & 17.24 \\ 
  \end{tabular}
\endgroup
\caption[optimal threshold, 1-tss and user/producer accuracy for all sites, Mahalanobis distance]{optimal threshold, 1-tss and user/producer accuracy for all sites, Mahalanobis distance} 
\end{table}


==> 3_Methodology/gridSearchAll_consecFix_mahl.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Thu Mar  9 23:13:26 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{lcl|ccccc}
 site & threshold & variable & 2 & 3 & 4 & 5 & 6 \\ 
  \hline
all & 17.24 & Mahl. dist. & 72.58 & 68.98 & 76.93 & 80.99 & 84.37 \\ 
  \end{tabular}
\endgroup
\caption[1-tss  all sites, Mahalanobis distance]{1-tss  all sites, Mahalanobis distance} 
\end{table}


==> 3_Methodology/gridSearchAll_consecVaries_cv_mahl.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Thu Mar  9 23:29:51 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{lll|ccccc|ccccc|ccccc}
 data & site & variable & 2 & 3 & 4 & 5 & 6 & 2 & 3 & 4 & 5 & 6 & 2 & 3 & 4 & 5 & 6 \\ 
  \hline
train & all & Mahl. dist. & 15.17 & 17.24 & 11.72 & 8.28 & 5.52 & 72.00 & 68.98 & 68.84 & 69.88 & 70.03 & 29.41 & 31.38 & 28.53 & 31.37 & 30.33 \\ 
  cv & all & Mahl. dist. & 15.17 & 17.24 & 11.72 & 8.28 & 5.52 & 74.94 & 70.17 & 68.96 & 72.90 & 72.16 & 29.42 & 31.34 & 29.91 & 30.34 & 30.27 \\ 
   \hline
\end{tabular}
\endgroup
\caption[optimal threshold, 1-tss and user/producer accuracy for all sites, Mahalanobis distance]{optimal threshold, 1-tss and user/producer accuracy for all sites, Mahalanobis distance} 
\end{table}


==> 3_Methodology/gridSearchAllbysite_consecVaries_mahl.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Thu Mar  9 21:02:46 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{ll|ccccc|ccccc}
 site & variable & 2 & 3 & 4 & 5 & 6 & 2 & 3 & 4 & 5 & 6 \\ 
  \hline
all & Mahl. dist. & 17.47 & 16.09 & 11.72 & 8.51 & 6.67 & 72.43 & 69.24 & 68.84 & 69.13 & 70.60 \\ 
  Sonora232 & Mahl. dist. & 17.47 & 16.09 & 11.72 & 8.51 & 6.67 & 99.39 & 88.61 & 95.65 & 102.46 & 98.08 \\ 
  Jalisco164 & Mahl. dist. & 17.47 & 16.09 & 11.72 & 8.51 & 6.67 & 38.32 & 38.91 & 38.45 & 32.99 & 38.45 \\ 
  Nayarit151 & Mahl. dist. & 17.47 & 16.09 & 11.72 & 8.51 & 6.67 & 49.89 & 44.37 & 40.94 & 43.97 & 38.07 \\ 
   \hline
Nayarit109 & Mahl. dist. & 17.47 & 16.09 & 11.72 & 8.51 & 6.67 & 45.83 & 56.15 & 51.19 & 41.67 & 46.43 \\ 
  Yucatan180 & Mahl. dist. & 17.47 & 16.09 & 11.72 & 8.51 & 6.67 & 97.89 & 68.93 & 73.81 & 70.23 & 71.88 \\ 
  QuintanaRoo100 & Mahl. dist. & 17.47 & 16.09 & 11.72 & 8.51 & 6.67 & 90.11 & 94.98 & 96.32 & 86.82 & 97.93 \\ 
  Michoacan98 & Mahl. dist. & 17.47 & 16.09 & 11.72 & 8.51 & 6.67 & 99.48 & 98.88 & 91.60 & 94.28 & 87.38 \\ 
  QuintanaRoo77 & Mahl. dist. & 17.47 & 16.09 & 11.72 & 8.51 & 6.67 & 72.91 & 75.33 & 65.07 & 61.65 & 70.14 \\ 
   \hline
Sonora74 & Mahl. dist. & 17.47 & 16.09 & 11.72 & 8.51 & 6.67 & 70.17 & 75.08 & 70.00 & 79.83 & 91.86 \\ 
  \end{tabular}
\endgroup
\caption{optimal threshold and 1-tss for each site (training data), Mahalanobis distance} 
\end{table}


==> 3_Methodology/gridSearch_consecFix1.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Tue Mar  7 21:21:18 2017
\begin{table}[ht]
\centering
\begin{tabular}{|l|rl|rrrrr|}
	  &           &          & \multicolumn{5}{|c|}{\# of consecutive violations}\\
 \hline	  
 site & threshold & variable & 2 & 3 & 4 & 5 & 6 \\ 
  \hline
Sonora232 & 0.080 & NIR\_reflectance & 86.293 & 70.448 & 58.785 & 66.891 & 69.523 \\ 
  Jalisco164 & 0.090 & NIR\_reflectance & 77.172 & 59.105 & 41.959 & 46.720 & 62.074 \\ 
  Nayarit151 & 0.080 & NIR\_reflectance & 81.818 & 41.288 & 23.918 & 47.998 & 47.808 \\ 
  Nayarit109 & 0.100 & NIR\_reflectance & 50.595 & 40.873 & 49.603 & 61.310 & 61.310 \\ 
   \hline
Yucatan180 & 0.200 & NDVI & 96.110 & 81.003 & 74.380 & 76.083 & 89.130 \\ 
  QuintanaRoo100 & 0.170 & NDVI & 86.416 & 87.504 & 81.799 & 85.210 & 100.268 \\ 
  Michoacan98 & 0.130 & NDVI & 84.778 & 77.490 & 58.780 & 65.404 & 63.072 \\ 
  QuintanaRoo77 & 0.180 & NDVI & 93.282 & 68.785 & 65.802 & 77.177 & 80.136 \\ 
  Sonora74 & 0.250 & NDVI & 62.373 & 61.356 & 60.678 & 70.678 & 90.339 \\ 
   \hline
\end{tabular}
\caption[$1-tss$ for each site trained separately with time series based on type of land-use change ]{$1-tss$ for each site trained separately with time series based on type of land-use change. Threshold corresponds to optimal threshold for 3 consecutive violations (training data)} 
\end{table}


==> 3_Methodology/gridSearch_consecFix_mahl.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Thu Mar  9 20:15:35 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{lcl|ccccc}
 site & threshold & variable & 2 & 3 & 4 & 5 & 6 \\ 
  \hline
Sonora232 & 17.241 & Mahl. dist. & 99.610 & 86.194 & 92.108 & 96.932 & 99.124 \\ 
  Jalisco164 & 13.103 & Mahl. dist. & 52.349 & 37.438 & 38.954 & 39.920 & 45.470 \\ 
  Nayarit151 & 11.724 & Mahl. dist. & 48.810 & 38.420 & 40.936 & 48.945 & 53.139 \\ 
  Nayarit109 & 8.276 & Mahl. dist. & 40.873 & 34.524 & 39.881 & 42.063 & 45.040 \\ 
   \hline
Yucatan180 & 18.621 & Mahl. dist. & 92.720 & 62.321 & 77.728 & 82.165 & 83.878 \\ 
  QuintanaRoo100 & 9.655 & Mahl. dist. & 91.317 & 92.791 & 80.727 & 84.942 & 94.981 \\ 
  Michoacan98 & 7.586 & Mahl. dist. & 92.306 & 76.467 & 77.503 & 89.888 & 92.353 \\ 
  QuintanaRoo77 & 13.103 & Mahl. dist. & 95.367 & 68.567 & 81.518 & 85.399 & 89.280 \\ 
  Sonora74 & 15.172 & Mahl. dist. & 79.661 & 65.932 & 82.034 & 91.356 & 91.017 \\ 
   \hline
\end{tabular}
\endgroup
\caption[1-tss for each site trained separately with Mahalanobis distance time series]{1-tss for each site trained separately with Mahalanobis distance time series} 
\end{table}


==> 3_Methodology/gridSearch_consecVaries1.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Tue Mar  7 22:13:03 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{|ll|rrrrr|rrrrr|rrrrr|}
     &           &  \multicolumn{5}{|c|}{optimal threshold} &  \multicolumn{5}{|c|}{1-tss} &  \multicolumn{5}{|c|}{user/producer accuracy}\\	
	\hline
 site & variable & 2 & 3 & 4 & 5 & 6 & 2 & 3 & 4 & 5 & 6 & 2 & 3 & 4 & 5 & 6 \\ 
  \hline
Sonora232 & NIR\_reflectance & 0.09 & 0.08 & 0.08 & 0.06 & 0.05 & 83.42 & 70.45 & 58.79 & 52.87 & 59.23 & 25.61 & 31.51 & 46.59 & 54.21 & 48.75 \\ 
  Jalisco164 & NIR\_reflectance & 0.13 & 0.11 & 0.09 & 0.06 & 0.05 & 54.41 & 49.37 & 41.96 & 36.69 & 33.73 & 46.20 & 54.10 & 63.98 & 63.81 & 64.81 \\ 
  Nayarit151 & NIR\_reflectance & 0.13 & 0.10 & 0.08 & 0.06 & 0.04 & 35.74 & 25.97 & 23.92 & 43.78 & 39.37 & 50.07 & 63.77 & 50.00 & 60.15 & 60.15 \\ 
  Nayarit109 & NIR\_reflectance & 0.13 & 0.10 & 0.10 & 0.06 & 0.05 & 37.50 & 40.87 & 49.60 & 51.19 & 47.82 & 59.62 & 38.89 & 41.27 & 39.61 & 37.04 \\ 
   \hline
Yucatan180 & NDVI & 0.28 & 0.22 & 0.20 & 0.12 & 0.12 & 82.65 & 78.84 & 74.38 & 69.10 & 79.34 & 32.58 & 23.69 & 22.42 & 11.86 & 11.91 \\ 
  QuintanaRoo100 & NDVI & 0.24 & 0.18 & 0.17 & 0.09 & 0.09 & 76.47 & 83.21 & 81.80 & 77.42 & 81.41 & 9.13 & 5.72 & 21.64 & 14.58 & 15.15 \\ 
  Michoacan98 & NDVI & 0.21 & 0.17 & 0.13 & 0.11 & 0.09 & 72.71 & 59.11 & 58.78 & 57.99 & 53.77 & 13.56 & 20.02 & 23.39 & 24.05 & 32.39 \\ 
  QuintanaRoo77 & NDVI & 0.24 & 0.19 & 0.18 & 0.13 & 0.11 & 81.54 & 68.25 & 65.80 & 53.24 & 54.62 & 9.43 & 16.72 & 15.39 & 27.05 & 25.66 \\ 
  Sonora74 & NDVI & 0.24 & 0.22 & 0.25 & 0.17 & 0.22 & 49.83 & 58.98 & 60.68 & 46.61 & 60.51 & 28.64 & 36.67 & 38.18 & 45.00 & 31.76 \\ 
   \hline
\end{tabular}
\endgroup
\caption[optimal threshold, 1-tss and user/producer accuracy for each site]{optimal threshold, 1-tss and user/producer accuracy for each site (training data)} 
\end{table}


==> 3_Methodology/gridSearch_consecVaries_cv1.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Tue Mar  7 22:27:01 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{|ll|rrrrr|rrrrr|rrrrr|}
\hline	
     &           &  \multicolumn{5}{|c|}{optimal threshold} &  \multicolumn{5}{|c|}{1-tss} &  \multicolumn{5}{|c|}{user/producer accuracy}\\	
 site & variable & 2 & 3 & 4 & 5 & 6 & 2 & 3 & 4 & 5 & 6 & 2 & 3 & 4 & 5 & 6 \\ 
  \hline
Sonora232 & NIR\_reflectance & 0.09 & 0.08 & 0.08 & 0.06 & 0.05 & 85.80 & 70.52 & 61.93 & 55.31 & 64.15 & 25.45 & 29.75 & 48.56 & 54.44 & 51.32 \\ 
  Jalisco164 & NIR\_reflectance & 0.13 & 0.11 & 0.09 & 0.06 & 0.05 & 63.76 & 56.27 & 43.30 & 36.87 & 33.53 & 48.10 & 58.65 & 62.74 & 65.22 & 64.61 \\ 
  Nayarit151 & NIR\_reflectance & 0.13 & 0.10 & 0.08 & 0.06 & 0.04 & 38.62 & 43.80 & 26.60 & 58.77 & 53.30 & 55.95 & 54.25 & 51.09 & 40.08 & 56.51 \\ 
  Nayarit109 & NIR\_reflectance & 0.13 & 0.10 & 0.10 & 0.06 & 0.05 & 53.34 & 45.23 & 52.10 & 53.50 & 55.63 & 61.03 & 46.98 & 43.51 & 48.10 & 38.17 \\ 
   \hline
Yucatan180 & NDVI & 0.28 & 0.22 & 0.20 & 0.12 & 0.12 & 83.70 & 89.51 & 78.32 & 72.44 & 90.49 & 33.86 & 23.49 & 21.77 & 11.97 & 12.57 \\ 
  QuintanaRoo100 & NDVI & 0.24 & 0.18 & 0.17 & 0.09 & 0.09 & 81.32 & 95.63 & 99.88 & 98.64 & 93.12 & 7.14 & 5.83 & 15.36 & 14.48 & 16.15 \\ 
  Michoacan98 & NDVI & 0.21 & 0.17 & 0.13 & 0.11 & 0.09 & 79.41 & 71.98 & 66.52 & 63.00 & 55.46 & 12.73 & 18.64 & 20.66 & 17.94 & 31.02 \\ 
  QuintanaRoo77 & NDVI & 0.24 & 0.19 & 0.18 & 0.13 & 0.11 & 107.88 & 76.82 & 77.71 & 71.46 & 61.50 & 8.33 & 11.51 & 13.89 & 21.85 & 21.67 \\ 
  Sonora74 & NDVI & 0.24 & 0.22 & 0.25 & 0.17 & 0.22 & 57.87 & 67.51 & 75.76 & 67.51 & 62.96 & 33.89 & 45.00 & 41.67 & 25.56 & 42.36 \\ 
   \hline
\end{tabular}
\endgroup
\caption[optimal threshold, 1-tss and user/producer accuracy for each site (cross validation)]{optimal threshold, 1-tss and user/producer accuracy for each site (cross validation)} 
\end{table}


==> 3_Methodology/gridSearch_consecVaries_cv_mahl.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Thu Mar  9 20:16:25 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{ll|ccccc|ccccc|ccccc}
 site & variable & 2 & 3 & 4 & 5 & 6 & 2 & 3 & 4 & 5 & 6 & 2 & 3 & 4 & 5 & 6 \\ 
  \hline
Sonora232 & Mahl. dist. & 9.66 & 17.24 & 5.52 & 13.10 & 5.52 & 98.87 & 86.21 & 96.03 & 96.84 & 97.36 & 19.13 & 20.06 & 18.85 & 15.99 & 15.50 \\ 
  Jalisco164 & Mahl. dist. & 16.55 & 13.10 & 12.41 & 8.28 & 5.52 & 37.92 & 39.18 & 38.68 & 31.93 & 36.80 & 67.07 & 67.93 & 64.02 & 68.67 & 69.69 \\ 
  Nayarit151 & Mahl. dist. & 13.79 & 11.72 & 11.72 & 10.34 & 8.28 & 45.93 & 44.39 & 45.25 & 41.76 & 38.74 & 53.67 & 59.26 & 58.80 & 57.87 & 65.00 \\ 
  Nayarit109 & Mahl. dist. & 9.66 & 8.28 & 8.97 & 8.97 & 3.45 & 48.91 & 42.11 & 58.91 & 51.50 & 43.51 & 50.19 & 43.73 & 41.16 & 51.94 & 49.07 \\ 
   \hline
Yucatan180 & Mahl. dist. & 20.00 & 18.62 & 12.41 & 13.10 & 8.28 & 97.13 & 69.91 & 76.99 & 77.37 & 73.98 & 43.23 & 40.17 & 32.60 & 24.97 & 22.24 \\ 
  QuintanaRoo100 & Mahl. dist. & 15.17 & 9.66 & 9.66 & 4.14 & 3.45 & 85.35 & 102.77 & 89.01 & 77.30 & 80.71 & 17.66 & 12.56 & 21.80 & 19.62 & 17.96 \\ 
  Michoacan98 & Mahl. dist. & 9.66 & 7.59 & 5.52 & 4.14 & 3.45 & 99.52 & 81.72 & 87.21 & 79.93 & 78.98 & 8.77 & 6.33 & 13.84 & 13.76 & 17.35 \\ 
  QuintanaRoo77 & Mahl. dist. & 19.31 & 13.10 & 9.66 & 5.52 & 5.52 & 81.54 & 87.53 & 67.82 & 68.62 & 79.32 & 26.69 & 22.38 & 15.00 & 21.46 & 14.09 \\ 
  Sonora74 & Mahl. dist. & 17.93 & 15.17 & 12.41 & 11.72 & 9.66 & 77.80 & 74.41 & 81.92 & 82.95 & 86.88 & 21.02 & 24.44 &  &  &  \\ 
   \hline
\end{tabular}
\endgroup
\caption[optimal threshold, 1-tss and user/producer accuracy for each site (cross validation), Mahalanobis distance]{optimal threshold, 1-tss and user/producer accuracy for each site (cross validation), Mahalanobis distance} 
\end{table}


==> 3_Methodology/gridSearch_consecVaries_mahl.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Thu Mar  9 20:16:17 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{ll|ccccc|ccccc|ccccc}
 site & variable & 2 & 3 & 4 & 5 & 6 & 2 & 3 & 4 & 5 & 6 & 2 & 3 & 4 & 5 & 6 \\ 
  \hline
Sonora232 & Mahl. dist. & 9.66 & 17.24 & 5.52 & 13.10 & 5.52 & 93.13 & 86.19 & 89.64 & 92.99 & 91.10 & 17.85 & 20.65 & 18.69 & 14.88 & 15.39 \\ 
  Jalisco164 & Mahl. dist. & 16.55 & 13.10 & 12.41 & 8.28 & 5.52 & 36.56 & 37.44 & 37.66 & 32.99 & 33.23 & 64.38 & 66.04 & 66.67 & 68.78 & 68.83 \\ 
  Nayarit151 & Mahl. dist. & 13.79 & 11.72 & 11.72 & 10.34 & 8.28 & 34.42 & 38.42 & 40.94 & 40.18 & 35.80 & 52.57 & 58.54 & 55.84 & 58.04 & 67.06 \\ 
  Nayarit109 & Mahl. dist. & 9.66 & 8.28 & 8.97 & 8.97 & 3.45 & 33.73 & 34.52 & 37.30 & 40.87 & 36.31 & 59.03 & 54.09 & 51.47 & 53.12 & 54.09 \\ 
   \hline
Yucatan180 & Mahl. dist. & 20.00 & 18.62 & 12.41 & 13.10 & 8.28 & 91.56 & 62.32 & 68.86 & 69.70 & 68.06 & 43.53 & 40.30 & 32.39 & 24.94 & 22.29 \\ 
  QuintanaRoo100 & Mahl. dist. & 15.17 & 9.66 & 9.66 & 4.14 & 3.45 & 82.02 & 92.79 & 80.73 & 78.57 & 85.92 & 13.17 & 5.72 & 24.44 & 19.05 & 10.32 \\ 
  Michoacan98 & Mahl. dist. & 9.66 & 7.59 & 5.52 & 4.14 & 3.45 & 81.07 & 76.47 & 74.37 & 71.65 & 64.71 & 9.02 & 6.48 & 13.15 & 13.15 & 17.88 \\ 
  QuintanaRoo77 & Mahl. dist. & 19.31 & 13.10 & 9.66 & 5.52 & 5.52 & 71.72 & 68.57 & 59.88 & 54.69 & 64.69 & 27.88 & 30.79 & 20.53 & 21.64 & 15.39 \\ 
  Sonora74 & Mahl. dist. & 17.93 & 15.17 & 12.41 & 11.72 & 9.66 & 69.15 & 65.93 & 66.78 & 75.59 & 74.75 & 20.00 & 23.82 & 19.09 & 10.56 & 21.11 \\ 
   \hline
\end{tabular}
\endgroup
\caption{optimal threshold, 1-tss and user/producer accuracy for each site (training data), Mahalanobis distance} 
\end{table}


==> 3_Methodology/landuseTable_Jalisco164.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Mar  5 15:55:50 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{rrrrrrrrrrrrrrrrrrrrr}
  & \begin{sideways} Temperate or sub-polar needleleaf forest \end{sideways} & \begin{sideways} Sub-polar taiga needleleaf forest \end{sideways} & \begin{sideways} Tropical or sub-tropical broadleaf evergreen forest \end{sideways} & \begin{sideways} Tropical or sub-tropical broadleaf deciduous forest \end{sideways} & \begin{sideways} Temperate or sub-polar broadleaf deciduous forest \end{sideways} & \begin{sideways} Mixed Forest \end{sideways} & \begin{sideways} Tropical or sub-tropical shrubland \end{sideways} & \begin{sideways} Temperate or sub-polar shrubland \end{sideways} & \begin{sideways} Tropical or sub-tropical grassland \end{sideways} & \begin{sideways} Temperate or sub-polar grassland \end{sideways} & \begin{sideways} Sub-polar or polar shrubland-lichen-moss \end{sideways} & \begin{sideways} Sub-polar or polar grassland-lichen-moss \end{sideways} & \begin{sideways} Sub-polar or polar barren-lichen-moss \end{sideways} & \begin{sideways} Wetland \end{sideways} & \begin{sideways} Cropland \end{sideways} & \begin{sideways} Barren Lands \end{sideways} & \begin{sideways} Urban and Built-up \end{sideways} & \begin{sideways} Water \end{sideways} & \begin{sideways} Snow and Ice \end{sideways} & \begin{sideways} Total \end{sideways} \\ 
  \hline
Temperate or sub-polar needleleaf forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    2 &    0 &    0 &    0 &    4 &    0 &    6 \\ 
  Sub-polar taiga needleleaf forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Tropical or sub-tropical broadleaf evergreen forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Tropical or sub-tropical broadleaf deciduous forest &    0 &    0 &    0 & 2631 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   21 &    1 &    0 &    0 &   58 &    0 & 2711 \\ 
  Temperate or sub-polar broadleaf deciduous forest &    0 &    0 &    0 &    3 &   96 &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    0 &   12 &    2 &    1 &    0 &   62 &    0 &  177 \\ 
  Mixed Forest &    0 &    0 &    0 &    0 &    0 &    4 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    4 \\ 
   \hline
Tropical or sub-tropical shrubland &    0 &    0 &    0 &    0 &    0 &    0 &   32 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   32 \\ 
  Temperate or sub-polar shrubland &    0 &    0 &    0 &    3 &    0 &    0 &    0 &  601 &    0 &    0 &    0 &    0 &    0 &    1 &    0 &    0 &    0 &    1 &    0 &  606 \\ 
  Tropical or sub-tropical grassland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Temperate or sub-polar grassland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   12 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   12 \\ 
  Sub-polar or polar shrubland-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar grassland-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar barren-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Wetland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Cropland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    0 &   19 & 1183 &    1 &    0 &   39 &    0 & 1243 \\ 
  Barren Lands &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   35 &    0 &   13 &    0 &   48 \\ 
  Urban and Built-up &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  130 &    3 &    0 &  133 \\ 
  Water &    0 &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    7 &    1 &    0 &    0 & 5019 &    0 & 5028 \\ 
  Snow and Ice &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
   \hline
Total &    0 &    0 &    0 & 2638 &   96 &    4 &   32 &  603 &    0 &   12 &    0 &    0 &    0 &   62 & 1187 &   37 &  130 & 5199 &    0 & 10000 \\ 
   \hline
\end{tabular}
\endgroup
\caption[NALCMS land-use distribution for site Jalisco164, 2005 and 2010.]{NALCMS land-use distribution for site Jalisco164, 2005 and 2010.} 
\end{table}


==> 3_Methodology/landuseTable_Michoacan98.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Mar  5 16:02:10 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{rrrrrrrrrrrrrrrrrrrrr}
  & \begin{sideways} Temperate or sub-polar needleleaf forest \end{sideways} & \begin{sideways} Sub-polar taiga needleleaf forest \end{sideways} & \begin{sideways} Tropical or sub-tropical broadleaf evergreen forest \end{sideways} & \begin{sideways} Tropical or sub-tropical broadleaf deciduous forest \end{sideways} & \begin{sideways} Temperate or sub-polar broadleaf deciduous forest \end{sideways} & \begin{sideways} Mixed Forest \end{sideways} & \begin{sideways} Tropical or sub-tropical shrubland \end{sideways} & \begin{sideways} Temperate or sub-polar shrubland \end{sideways} & \begin{sideways} Tropical or sub-tropical grassland \end{sideways} & \begin{sideways} Temperate or sub-polar grassland \end{sideways} & \begin{sideways} Sub-polar or polar shrubland-lichen-moss \end{sideways} & \begin{sideways} Sub-polar or polar grassland-lichen-moss \end{sideways} & \begin{sideways} Sub-polar or polar barren-lichen-moss \end{sideways} & \begin{sideways} Wetland \end{sideways} & \begin{sideways} Cropland \end{sideways} & \begin{sideways} Barren Lands \end{sideways} & \begin{sideways} Urban and Built-up \end{sideways} & \begin{sideways} Water \end{sideways} & \begin{sideways} Snow and Ice \end{sideways} & \begin{sideways} Total \end{sideways} \\ 
  \hline
Temperate or sub-polar needleleaf forest &   25 &    0 &    0 &    0 &    0 &    0 &    0 &    1 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    5 &    0 &    0 &   31 \\ 
  Sub-polar taiga needleleaf forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Tropical or sub-tropical broadleaf evergreen forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Tropical or sub-tropical broadleaf deciduous forest &    0 &    0 &    0 & 4669 &    0 &    0 &    0 &    0 &    6 &    0 &    0 &    0 &    0 &    0 &   14 &    0 &   37 &    0 &    0 & 4726 \\ 
  Temperate or sub-polar broadleaf deciduous forest &    0 &    0 &    0 &    1 &  243 &    0 &    0 &    4 &    0 &    0 &    0 &    0 &    0 &    0 &   12 &    0 &   19 &    0 &    0 &  279 \\ 
  Mixed Forest &    0 &    0 &    0 &    0 &    0 &  603 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  603 \\ 
   \hline
Tropical or sub-tropical shrubland &    0 &    0 &    0 &    0 &    0 &    0 &    9 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    9 \\ 
  Temperate or sub-polar shrubland &    3 &    0 &    0 &    6 &    0 &    0 &    0 & 1762 &    0 &    0 &    0 &    0 &    0 &    0 &    6 &    0 &   76 &    0 &    0 & 1853 \\ 
  Tropical or sub-tropical grassland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Temperate or sub-polar grassland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar shrubland-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar grassland-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar barren-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Wetland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Cropland &    1 &    0 &    0 &    2 &    1 &    0 &    0 &    1 &   12 &    0 &    0 &    0 &    0 &    0 & 2012 &    0 &  105 &    0 &    0 & 2134 \\ 
  Barren Lands &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Urban and Built-up &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  357 &    0 &    0 &  357 \\ 
  Water &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    8 &    0 &    8 \\ 
  Snow and Ice &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
   \hline
Total &   29 &    0 &    0 & 4678 &  244 &  603 &    9 & 1768 &   18 &    0 &    0 &    0 &    0 &    0 & 2044 &    0 &  599 &    8 &    0 & 10000 \\ 
   \hline
\end{tabular}
\endgroup
\caption[NALCMS land-use distribution for site Michoacan98, 2005 and 2010.]{NALCMS land-use distribution for site Michoacan98, 2005 and 2010.} 
\end{table}


==> 3_Methodology/landuseTable_Nayarit109.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Mar  5 15:59:41 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{rrrrrrrrrrrrrrrrrrrrr}
  & \begin{sideways} Temperate or sub-polar needleleaf forest \end{sideways} & \begin{sideways} Sub-polar taiga needleleaf forest \end{sideways} & \begin{sideways} Tropical or sub-tropical broadleaf evergreen forest \end{sideways} & \begin{sideways} Tropical or sub-tropical broadleaf deciduous forest \end{sideways} & \begin{sideways} Temperate or sub-polar broadleaf deciduous forest \end{sideways} & \begin{sideways} Mixed Forest \end{sideways} & \begin{sideways} Tropical or sub-tropical shrubland \end{sideways} & \begin{sideways} Temperate or sub-polar shrubland \end{sideways} & \begin{sideways} Tropical or sub-tropical grassland \end{sideways} & \begin{sideways} Temperate or sub-polar grassland \end{sideways} & \begin{sideways} Sub-polar or polar shrubland-lichen-moss \end{sideways} & \begin{sideways} Sub-polar or polar grassland-lichen-moss \end{sideways} & \begin{sideways} Sub-polar or polar barren-lichen-moss \end{sideways} & \begin{sideways} Wetland \end{sideways} & \begin{sideways} Cropland \end{sideways} & \begin{sideways} Barren Lands \end{sideways} & \begin{sideways} Urban and Built-up \end{sideways} & \begin{sideways} Water \end{sideways} & \begin{sideways} Snow and Ice \end{sideways} & \begin{sideways} Total \end{sideways} \\ 
  \hline
Temperate or sub-polar needleleaf forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar taiga needleleaf forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Tropical or sub-tropical broadleaf evergreen forest &    0 &    0 &    6 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    6 \\ 
  Tropical or sub-tropical broadleaf deciduous forest &    0 &    0 &    0 & 1658 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  109 &    0 & 1767 \\ 
  Temperate or sub-polar broadleaf deciduous forest &    0 &    0 &    0 &    0 &  337 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  337 \\ 
  Mixed Forest &    0 &    0 &    0 &    0 &    0 & 3266 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 & 3266 \\ 
   \hline
Tropical or sub-tropical shrubland &    0 &    0 &    0 &    0 &    0 &    0 &   17 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   17 \\ 
  Temperate or sub-polar shrubland &    0 &    0 &    0 &    4 &    0 &    0 &    0 & 3059 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    8 &    0 & 3071 \\ 
  Tropical or sub-tropical grassland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Temperate or sub-polar grassland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar shrubland-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar grassland-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar barren-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Wetland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Cropland &    0 &    0 &    0 &    6 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 & 1448 &    0 &    0 &   60 &    0 & 1514 \\ 
  Barren Lands &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    9 &    0 &    0 &    0 &    9 \\ 
  Urban and Built-up &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Water &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   13 &    0 &   13 \\ 
  Snow and Ice &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
   \hline
Total &    0 &    0 &    6 & 1668 &  337 & 3266 &   17 & 3059 &    0 &    0 &    0 &    0 &    0 &    0 & 1448 &    9 &    0 &  190 &    0 & 10000 \\ 
   \hline
\end{tabular}
\endgroup
\caption[NALCMS land-use distribution for site Nayarit109, 2005 and 2010.]{NALCMS land-use distribution for site Nayarit109, 2005 and 2010.} 
\end{table}


==> 3_Methodology/landuseTable_Nayarit151.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Mar  5 15:58:58 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{rrrrrrrrrrrrrrrrrrrrr}
  & \begin{sideways} Temperate or sub-polar needleleaf forest \end{sideways} & \begin{sideways} Sub-polar taiga needleleaf forest \end{sideways} & \begin{sideways} Tropical or sub-tropical broadleaf evergreen forest \end{sideways} & \begin{sideways} Tropical or sub-tropical broadleaf deciduous forest \end{sideways} & \begin{sideways} Temperate or sub-polar broadleaf deciduous forest \end{sideways} & \begin{sideways} Mixed Forest \end{sideways} & \begin{sideways} Tropical or sub-tropical shrubland \end{sideways} & \begin{sideways} Temperate or sub-polar shrubland \end{sideways} & \begin{sideways} Tropical or sub-tropical grassland \end{sideways} & \begin{sideways} Temperate or sub-polar grassland \end{sideways} & \begin{sideways} Sub-polar or polar shrubland-lichen-moss \end{sideways} & \begin{sideways} Sub-polar or polar grassland-lichen-moss \end{sideways} & \begin{sideways} Sub-polar or polar barren-lichen-moss \end{sideways} & \begin{sideways} Wetland \end{sideways} & \begin{sideways} Cropland \end{sideways} & \begin{sideways} Barren Lands \end{sideways} & \begin{sideways} Urban and Built-up \end{sideways} & \begin{sideways} Water \end{sideways} & \begin{sideways} Snow and Ice \end{sideways} & \begin{sideways} Total \end{sideways} \\ 
  \hline
Temperate or sub-polar needleleaf forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar taiga needleleaf forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Tropical or sub-tropical broadleaf evergreen forest &    0 &    0 &  170 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  170 \\ 
  Tropical or sub-tropical broadleaf deciduous forest &    0 &    0 &    0 & 5876 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  151 &    0 & 6027 \\ 
  Temperate or sub-polar broadleaf deciduous forest &    0 &    0 &    0 &    0 &  223 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  223 \\ 
  Mixed Forest &    0 &    0 &    0 &    0 &    0 &  170 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  170 \\ 
   \hline
Tropical or sub-tropical shrubland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    7 &    0 &    0 &    0 &    0 &    7 \\ 
  Temperate or sub-polar shrubland &    0 &    0 &    0 &    0 &    0 &    0 &    0 & 1278 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 & 1278 \\ 
  Tropical or sub-tropical grassland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Temperate or sub-polar grassland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar shrubland-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar grassland-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar barren-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Wetland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Cropland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 & 1873 &    0 &    0 &   20 &    0 & 1893 \\ 
  Barren Lands &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    9 &    0 &    0 &    5 &    0 &   14 \\ 
  Urban and Built-up &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Water &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  218 &    0 &  218 \\ 
  Snow and Ice &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
   \hline
Total &    0 &    0 &  170 & 5876 &  223 &  170 &    0 & 1278 &    0 &    0 &    0 &    0 &    0 &    0 & 1889 &    0 &    0 &  394 &    0 & 10000 \\ 
   \hline
\end{tabular}
\endgroup
\caption[NALCMS land-use distribution for site Nayarit151, 2005 and 2010.]{NALCMS land-use distribution for site Nayarit151, 2005 and 2010.} 
\end{table}


==> 3_Methodology/landuseTable_QuintanaRoo100.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Mar  5 16:01:40 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{rrrrrrrrrrrrrrrrrrrrr}
  & \begin{sideways} Temperate or sub-polar needleleaf forest \end{sideways} & \begin{sideways} Sub-polar taiga needleleaf forest \end{sideways} & \begin{sideways} Tropical or sub-tropical broadleaf evergreen forest \end{sideways} & \begin{sideways} Tropical or sub-tropical broadleaf deciduous forest \end{sideways} & \begin{sideways} Temperate or sub-polar broadleaf deciduous forest \end{sideways} & \begin{sideways} Mixed Forest \end{sideways} & \begin{sideways} Tropical or sub-tropical shrubland \end{sideways} & \begin{sideways} Temperate or sub-polar shrubland \end{sideways} & \begin{sideways} Tropical or sub-tropical grassland \end{sideways} & \begin{sideways} Temperate or sub-polar grassland \end{sideways} & \begin{sideways} Sub-polar or polar shrubland-lichen-moss \end{sideways} & \begin{sideways} Sub-polar or polar grassland-lichen-moss \end{sideways} & \begin{sideways} Sub-polar or polar barren-lichen-moss \end{sideways} & \begin{sideways} Wetland \end{sideways} & \begin{sideways} Cropland \end{sideways} & \begin{sideways} Barren Lands \end{sideways} & \begin{sideways} Urban and Built-up \end{sideways} & \begin{sideways} Water \end{sideways} & \begin{sideways} Snow and Ice \end{sideways} & \begin{sideways} Total \end{sideways} \\ 
  \hline
Temperate or sub-polar needleleaf forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar taiga needleleaf forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Tropical or sub-tropical broadleaf evergreen forest &    0 &    0 & 4286 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   90 &    0 &   10 &    0 &    0 & 4386 \\ 
  Tropical or sub-tropical broadleaf deciduous forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Temperate or sub-polar broadleaf deciduous forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Mixed Forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
   \hline
Tropical or sub-tropical shrubland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Temperate or sub-polar shrubland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Tropical or sub-tropical grassland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Temperate or sub-polar grassland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar shrubland-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar grassland-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar barren-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Wetland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  674 &    0 &    0 &    0 &    0 &    0 &  674 \\ 
  Cropland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 & 2361 &    0 &   28 &    2 &    0 & 2391 \\ 
  Barren Lands &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    4 &    0 &   20 &    0 &    1 &    0 &   25 \\ 
  Urban and Built-up &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  313 &    0 &    0 &  313 \\ 
  Water &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    2 &    0 &    0 &    0 &  295 &    0 &  297 \\ 
  Snow and Ice &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
   \hline
Total &    0 &    0 & 4286 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  680 & 2451 &   20 &  351 &  298 &    0 & 8086 \\ 
   \hline
\end{tabular}
\endgroup
\caption[NALCMS land-use distribution for site QuintanaRoo100, 2005 and 2010.]{NALCMS land-use distribution for site QuintanaRoo100, 2005 and 2010.} 
\end{table}


==> 3_Methodology/landuseTable_QuintanaRoo77.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Mar  5 16:02:46 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{rrrrrrrrrrrrrrrrrrrrr}
  & \begin{sideways} Temperate or sub-polar needleleaf forest \end{sideways} & \begin{sideways} Sub-polar taiga needleleaf forest \end{sideways} & \begin{sideways} Tropical or sub-tropical broadleaf evergreen forest \end{sideways} & \begin{sideways} Tropical or sub-tropical broadleaf deciduous forest \end{sideways} & \begin{sideways} Temperate or sub-polar broadleaf deciduous forest \end{sideways} & \begin{sideways} Mixed Forest \end{sideways} & \begin{sideways} Tropical or sub-tropical shrubland \end{sideways} & \begin{sideways} Temperate or sub-polar shrubland \end{sideways} & \begin{sideways} Tropical or sub-tropical grassland \end{sideways} & \begin{sideways} Temperate or sub-polar grassland \end{sideways} & \begin{sideways} Sub-polar or polar shrubland-lichen-moss \end{sideways} & \begin{sideways} Sub-polar or polar grassland-lichen-moss \end{sideways} & \begin{sideways} Sub-polar or polar barren-lichen-moss \end{sideways} & \begin{sideways} Wetland \end{sideways} & \begin{sideways} Cropland \end{sideways} & \begin{sideways} Barren Lands \end{sideways} & \begin{sideways} Urban and Built-up \end{sideways} & \begin{sideways} Water \end{sideways} & \begin{sideways} Snow and Ice \end{sideways} & \begin{sideways} Total \end{sideways} \\ 
  \hline
Temperate or sub-polar needleleaf forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar taiga needleleaf forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Tropical or sub-tropical broadleaf evergreen forest &    0 &    0 & 2975 &    0 &    0 &    0 &    0 &    0 &    5 &    0 &    0 &    0 &    0 &    0 &   37 &    0 &   35 &    0 &    0 & 3052 \\ 
  Tropical or sub-tropical broadleaf deciduous forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Temperate or sub-polar broadleaf deciduous forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Mixed Forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
   \hline
Tropical or sub-tropical shrubland &    0 &    0 &    0 &    0 &    0 &    0 &    4 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    4 \\ 
  Temperate or sub-polar shrubland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Tropical or sub-tropical grassland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Temperate or sub-polar grassland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar shrubland-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar grassland-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar barren-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Wetland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  169 &    0 &    0 &    0 &    0 &    0 &  169 \\ 
  Cropland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    7 &    0 &    0 &    0 &    0 &    1 &  952 &    0 &   60 &    0 &    0 & 1020 \\ 
  Barren Lands &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Urban and Built-up &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  313 &    0 &    0 &  313 \\ 
  Water &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    1 &    0 &    1 \\ 
  Snow and Ice &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
   \hline
Total &    0 &    0 & 2975 &    0 &    0 &    0 &    4 &    0 &   12 &    0 &    0 &    0 &    0 &  170 &  989 &    0 &  408 &    1 &    0 & 4559 \\ 
   \hline
\end{tabular}
\endgroup
\caption[NALCMS land-use distribution for site QuintanaRoo77, 2005 and 2010.]{NALCMS land-use distribution for site QuintanaRoo77, 2005 and 2010.} 
\end{table}


==> 3_Methodology/landuseTable_Sonora74.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
% Sun Mar  5 16:03:51 2017
\begin{table}[ht]
\centering
\begingroup\tiny
\begin{tabular}{rrrrrrrrrrrrrrrrrrrrr}
  & \begin{sideways} Temperate or sub-polar needleleaf forest \end{sideways} & \begin{sideways} Sub-polar taiga needleleaf forest \end{sideways} & \begin{sideways} Tropical or sub-tropical broadleaf evergreen forest \end{sideways} & \begin{sideways} Tropical or sub-tropical broadleaf deciduous forest \end{sideways} & \begin{sideways} Temperate or sub-polar broadleaf deciduous forest \end{sideways} & \begin{sideways} Mixed Forest \end{sideways} & \begin{sideways} Tropical or sub-tropical shrubland \end{sideways} & \begin{sideways} Temperate or sub-polar shrubland \end{sideways} & \begin{sideways} Tropical or sub-tropical grassland \end{sideways} & \begin{sideways} Temperate or sub-polar grassland \end{sideways} & \begin{sideways} Sub-polar or polar shrubland-lichen-moss \end{sideways} & \begin{sideways} Sub-polar or polar grassland-lichen-moss \end{sideways} & \begin{sideways} Sub-polar or polar barren-lichen-moss \end{sideways} & \begin{sideways} Wetland \end{sideways} & \begin{sideways} Cropland \end{sideways} & \begin{sideways} Barren Lands \end{sideways} & \begin{sideways} Urban and Built-up \end{sideways} & \begin{sideways} Water \end{sideways} & \begin{sideways} Snow and Ice \end{sideways} & \begin{sideways} Total \end{sideways} \\ 
  \hline
Temperate or sub-polar needleleaf forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar taiga needleleaf forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Tropical or sub-tropical broadleaf evergreen forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Tropical or sub-tropical broadleaf deciduous forest &    0 &    0 &    0 & 8788 &    0 &    0 &   16 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   57 &    0 &    1 &    0 & 8862 \\ 
  Temperate or sub-polar broadleaf deciduous forest &    0 &    0 &    0 &    0 &   16 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   16 \\ 
  Mixed Forest &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
   \hline
Tropical or sub-tropical shrubland &    0 &    0 &    0 &    0 &    0 &    0 &   22 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &   22 \\ 
  Temperate or sub-polar shrubland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Tropical or sub-tropical grassland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Temperate or sub-polar grassland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar shrubland-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar grassland-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Sub-polar or polar barren-lichen-moss &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Wetland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Cropland &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  824 &    0 &    0 &    0 &    0 &  824 \\ 
  Barren Lands &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
  Urban and Built-up &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    5 &    0 &    0 &    5 \\ 
  Water &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  271 &    0 &  271 \\ 
  Snow and Ice &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &    0 \\ 
   \hline
Total &    0 &    0 &    0 & 8788 &   16 &    0 &   38 &    0 &    0 &    0 &    0 &    0 &    0 &    0 &  824 &   57 &    5 &  272 &    0 & 10000 \\ 
   \hline
\end{tabular}
\endgroup
\caption[NALCMS land-use distribution for site Sonora74, 2005 and 2010.]{NALCMS land-use distribution for site Sonora74, 2005 and 2010.} 
\end{table}


==> 3_Methodology/simAnn_consecFix1.tex <==
% latex table generated in R 3.3.2 by xtable 1.8-2 package
% Wed Mar  8 21:28:51 2017
\begin{table}[ht]
\centering
\begin{tabular}{|lrrl|rrrrr||}
  \hline
site & threshold NIR & threshold NDVI & variable & 2 & 3 & 4 & 5 & 6 \\ 
  \hline
all & 0.120 & 0.241 & both & 76.562 & 71.539 & 76.396 & 77.540 & 82.348 \\ 
   \hline
Sonora232 & 0.120 & 0.241 & both & 97.452 & 93.676 & 87.947 & 89.477 & 92.108 \\ 
  Jalisco164 & 0.120 & 0.241 & both & 71.188 & 39.699 & 46.303 & 45.470 & 55.275 \\ 
  Nayarit151 & 0.120 & 0.241 & both & 49.324 & 35.579 & 44.372 & 53.328 & 57.711 \\ 
  Nayarit109 & 0.120 & 0.241 & both & 35.317 & 45.437 & 67.857 & 72.421 & 77.976 \\ 
   \hline
Yucatan180 & 0.120 & 0.241 & both & 99.774 & 87.458 & 90.228 & 84.977 & 91.421 \\ 
  QuintanaRoo100 & 0.120 & 0.241 & both & 92.821 & 103.485 & 100.536 & 100.268 & 100.000 \\ 
  Michoacan98 & 0.120 & 0.241 & both & 89.542 & 89.675 & 94.260 & 93.489 & 93.103 \\ 
  QuintanaRoo77 & 0.120 & 0.241 & both & 86.030 & 91.657 & 101.188 & 103.687 & 101.382 \\ 
  Sonora74 & 0.120 & 0.241 & both & 62.712 & 68.305 & 61.695 & 61.356 & 81.356 \\ 
   \hline
\end{tabular}
\caption[1-tss for all sites using thresholds trained simultaneously with simulated annealing]{1-tss for all sites using thresholds trained simultaneously with simulated annealing} 
\end{table}

